System Resilience through Health Monitoring and Reconfiguration

We demonstrate an end-to-end framework to improve the resilience of man-made systems to unforeseen events. The framework is based on a physics-based digital twin model and three modules tasked with real-time fault diagnosis, prognostics and reconfiguration. The fault diagnosis module uses model-based diagnosis algorithms to detect and isolate faults and generates interventions in the system to disambiguate uncertain diagnosis solutions. We scale up the fault diagnosis algorithm to the required real-time performance through the use of parallelization and surrogate models of the physics-based digital twin. The prognostics module tracks the fault progressions and trains the online degradation models to compute remaining useful life of system components. In addition, we use the degradation models to assess the impact of the fault progression on the operational requirements. The reconfiguration module uses PDDL-based planning endowed with semantic attachments to adjust the system controls so that the fault impact on the system operation is minimized. We define a resilience metric and use the example of a fuel system model to demonstrate how the metric improves with our framework.

==> open_challenges.tex <==
\section{Open challenges}
Scalability (Alex)

Diagnosis of multiple faults (Johan)

Automatic generation of surrogate models for planning. 
Modelica models have XML descriptions that contain information about the structure and dynamics of the system which can be used to define planning domain features and constraints (e.g., bounds on variable values). Such information can be used in the construction of PDDL models. Causality properties (e.g., input/output properties), or variable type (discrete or continuous) can also be used for building PDDL models.

There is also a need for improved search performance. Here we demonstrated a new class of PDDL+ planning problems using complex semantic attachments. Such tasks call for a new type of heuristics that can reason with the structure and design of the system as well as the location of faults. Intelligent domain-independent heuristics containing system composition and design information can bring about a wave of novel planning-based aproaches to self-reconfigurable machines and agents.
